Enhancing Bitcoin Security and Performance with Strong Consistency via Collective Signing

While showing great promise, Bitcoin requires users to wait tens of minutes for transactions to commit, and even then, offering only probabilistic guarantees. This paper introduces ByzCoin, a novel Byzantine consensus protocol that leverages scalable collective signing to commit Bitcoin transactions irreversibly within seconds. ByzCoin achieves Byzantine consensus while preserving Bitcoin's open membership by dynamically forming hash power-proportionate consensus groups that represent recently-successful block miners. ByzCoin employs communication trees to optimize transaction commitment and verification under normal operation while guaranteeing safety and liveness under Byzantine faults, up to a near-optimal tolerance of f faulty group members among 3f + 2 total. ByzCoin mitigates double spending and selfish mining attacks by producing collectively signed transaction blocks within one minute of transaction submission. Tree-structured communication further reduces this latency to less than 30 seconds. Due to these optimizations, ByzCoin achieves a throughput higher than PayPal currently handles, with a confirmation latency of 15-20 seconds.

==> appA.tex <==
\section*{Appendix A~: Bitcoin propagation algorithm}

To facilitate scalability in Bitcoin, messages are propagated 
in the Bitcoin network via an advertisement based model. 
If node A receives a new block, A verifies that the object is correct 
and then advertises it to his connection (e.g node B) 
with an inv (inventory) message like Figure~\ref{fig:bitcoin_prop.eps}. 
This helps minimize the bandwidth usage since inv messages are a lot smaller than the real block.
Only if
node B has not previously received the block advertised by the inv
message, B will request the block from A with a getdata request.
Following the protocol, node A will subsequently respond
with the block. 
This practice limits the bandwidth consumption in the network 
since B only gets inv messages from all his connection 
but request the full block only from one peer. 
The nodes first receive the header and then the transactions of the block 
so that they can verify the header first 
and reject it quickly if it has a wrong proof-of-work.

\diagramscale{Bitcoin Propagation Algorithm}{bitcoin_prop.eps}{0.5}


==> appB.tex <==
\section*{Appendix A~: Selfish mining elimination in \coinname{}}

If the smallest hash wins is used then a selfish miner can be lucky 
and get a smaller than needed hash of the block. 
For example, the target can be $10$ leading zero bits 
but the miner finds a block with $12$ leading zero bits ($\frac{1}{2^2}$ probability).
Then this block has a $87,5\%$ chance of winning a potential fork, 
thus it might be better to keep it hidden and try to find a second block on it.
We prove that a miner with $25\%$ computing power can get bigger revenue then.

We note as $c$ the computing power of an attacker 
and $G$ the chance to put a block in the block chain and gain the reward. 
If the attacker is not selfishly mining then $G=c$. 
If the attacker selfishly mines then 
\begin{equation} \label{eq: eq} 
G= c*\left[\left(1-\frac{1}{2^n}\right)+\frac{1}{2^n}*\left(1-2^{-n-1}\right)*\left(1+G\right)\right]
\end{equation}
where $n$ is the additional zero bits the selfish miner's block have. 
The probability that the miner finds a block with less than $n$ additional 
zero-bits is $\left(1-\frac{1}{2^n}\right)$. 
In this case the attacker decides that the block is not worth the risk 
and publishes it to get the reward.
If on the other hand the block is good enough ($\frac{1}{2^n}$ probability)
the attacker keeps it hidden and mines on it. 
If another miner creates a conflicting block the the attacker has $\left(1-2^{-n-1}\right)$
probability of winning the conflict, 
since he loses only if the other miners has found a block with $n+1$ more zeros than the target. 
If the miner wins he gets the block reward plus the chance to gain 
from the hidden blockchain (1 for the win of the conflict 
and G for the possibility to win the next block).
 
For $c=0.25$ and $n = 2$, $G=0.2562$ which means that 
if a selfish miner with $25\%$ computing power tries to selfish mine  
he can get $25,62\%$ of the revenue. 
As n increases the minimum c decreases, thus almost everyone can try to selfish mine. 
Furthermore as c increases the total percentage of the revenue increases, 
thus mining in pools is favorable. 
This results leads to the same problem as the original selfish mining paper.

In \coinname{} there is only $50\%$ chance of winning a block 
and in the case of loosing all hidden work is wasted. 
The expected wins of a selfish miner can also be calculated by equation~\cref{eq: eq} when $n=0$. 
Then we can see that in order for $G > c $ we need $c  > 1 $ i.e the attacker needs to have more than 100\% of the computing power, which is impossible.



==> implementation.tex <==
\section{Prototype Implementation}  \label{sec:impl}

We have built and evaluated a working prototype of \coinname{} 
layered upon the CoSi implementation which is written in Go~\cite{Go} 
and is available at https://github.com/DeDiS.
The \coinname{} prototype currently implements both normal and tree-based
collective block signing as described above.
We evaluated the \coinname{} implementation with Schnorr
signatures implemented over the Ed25519 curve~\cite{bernstein12highspeed}.

The \coinname{} is implemented on top of the Signer layer of CoSi. 
There are also clients parsing real Bitcoin transactions 
and sending them to the servers so that they can create blocks. 
Both microblocks and keyblocks are fully transmitted 
and collectively signed through the tree and are returned, 
together with the proof, to the clients upon request. 
The verification of the block header is implemented 
and the verification of the transactions inside the block is emulated 
because the low available Cores and RAM (1 quad-core and 16GB per machine where we run up to 25 hosts) of the testbed, 
would impose an unrealistic bottleneck. 
The same practice is proposed in Shadow Bitcoin~\cite{miller2015shadow}. 
We base our emulation both on measurements\cite{gervais2015tampering} of the average block verification delays (around 200ms for 500MB block) 
and the claims of Bitcoin Developers~\cite{scaling}. 
We simulate a linear increase of this delay based on the number of transactions included in the block.
% We are aware that this is not always true, but since the leader proposes the blocks to be signed it is his job to choose appropriate transactions based on their fees as mentioned in Section \ref{sec:Fees}. 
Because of the communication pattern of \coinname , 
the transaction verification cost delays only the leaf nodes. 
By the time the leaf nodes finish the block verification 
and send their vote back to their parents, 
all other tree nodes would have already finished the verification 
and can immediately proceed. 
For this reason the primary delay factor is the transmission of the blocks 
that needs to be done $\log N$ times. 
Finally the Bitcoin-core developers state~\cite{scaling} 
that as far as transaction verification is concerned,
Bitcoin nodes can handle up to 4000 TPS, 
hence the less than 1000 TPS that \coinname{} achieves 
will not be affected by the transaction verification delay.
\com{
\paragraph{Implementation Improvements.} 
Collective Signing~\cite{syta15decentralizing} is done 
in four different phases per round, 
namely Announce phase, Response phase, Challenge phase and Commit phase.
In the \coinname{} the Announce and Commit phases of the CoSi protocol are not used 
since the proposed messages (the block in the prepare round and the proof-of-acceptance in the commit round) 
can be sent to the signers on the Challenge phase. 
This allows for the intersection of the two rounds 
so that the announce/commit phases of the 
\coinname's commit round are piggybacked on the challenge 
and response messages of the \coinname's prepare round. 
This pipeline allows for a reduction of latency (one less round-trip) 

Looking into the normal execution of \coinname{} this pipeline 
can be extended so that an optimal throughput 
of one signed microblock per round-trip is produced  on \coinname . 
A sample execution can be seen in \cref{tab:byzcoin-pipeline}.

%\diagramscale{Maximum Throughput achieved in \coinname{}: An/Co is the Announce-Commit round-trip of CoSi and Ch/Re the Challenge-Response, B(k) is the microblock with height k and the arrows show dependency between the B(k) prepare round and the other rounds. On every round-trip there is a commit block round finishing. \xxx{B(k) notation is only used in this Figure} }{pipeline.eps}{0.25}

\begin{table}[ht]
    \centering
    \scriptsize
    \begin{tabular}{llccccc}
        \toprule
                                   &            & $t_i$ & $t_{i+1}$ & $t_{i+2}$ & $t_{i+3}$ & $t_{i+4}$ \\
        \midrule
        \multirow{2}{*}{$B_k$}     &  prepare   & An/Co & Ch/Re & & & \\
                                   &  commit    & & An/Co & Ch/Re & & \\
        \midrule
        \multirow{2}{*}{$B_{k+1}$} &  prepare   & & An/Co & Ch/Re & & \\
                                   &  commit    & & & An/Co & Ch/Re & \\
        \midrule
        \multirow{2}{*}{$B_{k+2}$} &  prepare   & & & An/Co & Ch/Re & \\
                                   &  commit    & & & & An/Co & Ch/Re \\
        \bottomrule
    \end{tabular}
    \caption{\coinname pipelining for maximum transaction-throughput; $B_k$
    denotes the microblock signed in round $k$, An/Co the Announce-Commit and
    Ch/Re the Challenge-Response round-trips of CoSi}
    \label{tab:byzcoin-pipeline}
\end{table}
}




==> tree.tex <==


\subsection{Fault Tolerance} 

\subsubsection{Leader Unavailability}

\xxx{ This discussion should be earlier, somewhere before the Bitcoin-NG part,
	probably around where view changes are (should be) discussed in detail.
	That in turn should be not far from where the membership selection
	protocol is introduced and discussed in detail.
}

In \coinname{} there is the possibility that a Byzantine leader stops creating micro-blocks 
or creates wrong ones. 
In order to preserve liveness and allow the system to make progress 
\coinname{} has a standard PBFT-style~\cite{castro1999practical} view-change protocol.

Every witness resets a timer when signing one block. 
If the timer of the witness expires, 
or the leader behaves maliciously (proposed wrong blocks), 
the witness decides that the leader is faulty and broadcasts a view-change message to everyone. 
 Afterwards he stops accepting blocks from the current leader. 
 When $2f+1$ nodes have send the view-change message the next leader takes over. 
The new view is simply going to be the last view that worked correctly. 
So if the leader of the keyblock $i$ fails, the next leader is going to be again the miner of keyblock $i-1$. 
 When the new leader takes over the first micro-block has to be consistent with the current state of the blockchain 
 and as we show in Section \ref{sec:3f+2} it needs $2f+2$ supporting votes.

\subsubsection{Tree Fault Tolerance}\label{sec:FT}

\xxx{ CoSi is designed with fault-tolerance in mind! 
	Just not fault tolerance of the leader; is that what you mean here?
	clarify. 
	What is the fault tolerance problem this subseciton is talking about? 
	churn among the current consensus group? 
	If so, pick a clearer subsection title indicating that.
}

At the beginning of this section we mentioned that CoSi is not design with 
fault-tolerance in mind, but with scalability. 
There are two different mechanisms proposed in order to allow for substantial fault-tolerance in the original paper~\cite{syta15decentralizing}. 
Furthermore the strict membership requirements, 
the frequent tree changes of \coinname{} 
and the multiple virtual miners per real miner 
increase the difficulty of a malicious attacker with less than 33\% of the total computing power to attack the system. 
However, a security analysis must assume that a Byzantine adversary 
is able to get the correct nodes of the \coinname{} signing tree 
so that it can compromise the Liveness of the system by a simple DoS of his 
virtual miners (Safety is always optimal at $f$ tolerated faults out of $3f+2$ virtual miners). 
To mitigate that we focus on the latest research done in Byzantine Fault Tolerance.

For this reason we use the ideas of adversary oriented computing~\cite{guerraoui2010next} to achieve the optimal Liveness guarantees of a distributed system. 
This means that in a system with $3f+2$ nodes we can get $f$ faults ($33\%$ of computing power).

\xxx{ I really don't understand what point this paragraph is trying to make.} 
Guerraoui et al. define a new abstraction in State Machine Replication~\cite{schneider1990implementing} so that BFT-SMR is only a subset of what can be used.
 They achieve that, by defining the protocol needed to be deployed based on the adversary the system is facing. 
 An adversary is not necessarily an intelligent one. 
 A congested network with high loss rate is also considered as an adversary for example. 
 The strongest adversary is the Byzantine.

After defining the adversaries, they state that one-size fits all protocols have a high implementation complexity 
and degrade normal case performance in order to withstand Byzantine faults. 
For this reason, a suite of protocols should be deployed which provide incremental Safety guarantees. 
If one protocol is too weak a stronger one is deployed.

With the same ideas in mind, we redefine \coinname{} 
so that the tree communication pattern is only a normal case performance optimization 
that can withstand most malicious attacks. 
However, when the the Liveness of the tree \coinname{} is compromised 
the system should not halt, the leader can decide to get back to the non-tree based communication 
until the end of his era.
The leader detects that the tree has failed by broadcasting the hash of the block he proposes after sending it through the tree. 
The nodes reply when they get the block from the tree with an ACK. 
With these messages the leader knows when he should revert to the non-tree \coinname{}
before the witnesses assume that he is faulty and try to view-change.
The possibility that the next leader faces the same problem is low, 
especially if the branching factor of the tree is high, 
but he can deploy the same protocol until the adversary looses power. 

\xxx{ In general, this whole subsection up to this point
	is currently so unclear as to be useless. 
	If it's trying to make an important point,
	we need to figure out what that is and completely rewrite it.
}

\subsubsection{Membership Churn and BFT}\label{sec:3f+2}

After a new leader is elected the system needs to ensure that 
the first microblock of the new leader points to the last microblock of the previous leader. 
Having $2f+1$ supporting votes is not enough. 
This happens because there is the possibility 
that an honest node lost membership when the new epoch started. 
This means that the system now in the worst case has $f$ Byzantine nodes,
$f$ honest nodes that are up to date, $f$ slow nodes that have a stale view of the blockchain 
and the new leader that might also have a stale view. 
This can lead to the leader proposing a new microblock 
ignoring some signed microblocks and getting $2f+1$ support (stale+Byzantine+his own). 
For this reason the first micro-block of an era need $2f+2$ supporting signatures. 
If the leader is unable to get them this means that he needs to synchronize with the system,
\ie, he needs to find the latest signed micro-block from the previous roster. 
For this reason he asks all the nodes in his roster plus the node that lost membership 
to sign a latest checkpoint message containing the hash of the last microblock.
In this point of time the system has $3f+2$ ($3f+1$ of the previous roster plus the leader) members 
and needs $2f+1$ honest nodes to verify the checkpoint 
plus an honest leader to accept it (a Byzantine leader will be the $f+1$ fault and compromise Liveness). 
Thus, \coinname{} can tolerate $f$ fails in $3f+2$ nodes at this point of time. 

